Proofs about Network Communication: For Humans and Machines

Many concurrent and distributed systems are safety-critical and therefore have to provide a high degree of assurance. Important properties of such systems are frequently proved on the specification level, but implementations typically deviate from specifications for practical reasons. Machine-checked proofs of bisimilarity statements are often useful for guaranteeing that properties of specifications carry over to implementations. In this paper, we present a way of conducting such proofs with a focus on network communication. The proofs resulting from our approach are not just machine-checked but also intelligible for humans.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{C. Aubert, C. Di Giusto, S. Fowler \& L. Safina (Eds.):\\
16th Interaction and Concurrency Experience (ICE 2023)\\
EPTCS 383, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.383.1}{10.4204/EPTCS.383.1}}
\pdfoutput=1

